Fair Classification under Covariate Shift and Missing Protected Attribute -- an Investigation using Related Features

This study investigated the problem of fair classification under Covariate Shift and missing protected attribute using a simple approach based on the use of importance-weights to handle covariate-shift and, Related Features arXiv:2104.14537 to handle missing protected attribute.

==> tmp.tex <==
% Temporary content.
